Boosting Top Partner Searches in Composite Higgs Models

Fermionic third generation top partners are generic in composite Higgs models. They are likely to decay into third generation quarks and electroweak bosons. We propose a novel cut-and-count-style analysis in which we cross correlate the model-dependent single and model-independent pair production processes for the top partners $X_{5/3}$ and $B$. In the class of composite Higgs models we study, $X_{5/3}$ is very special as it is the lightest exotic fermion. A constraint on the mass of $X_{5/3}$ directly extends to constrains on all top partner masses. By combining jet substructure methods with conventional reconstruction techniques we show that in this kind of final state a smooth interpolation between the boosted and unboosted regime is possible. We find that a reinterpretation of existing searches can improve bounds on the parameter space of composite Higgs models. Further, at 8 TeV a combined search for $X_{5/3}$ and $B$ in the $l+\rm{jets}$ final state can be more sensitive than a search involving same-sign dileptons.

==> application.tex <==

%%%%%%%%%%%%%%%%%%%%%%
%  Applications
%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
\begin{center}
\epsfxsize=0.48\textwidth\epsfbox{c1VSmassljetsCUTCOUNTy3.pdf}
\epsfxsize=0.48\textwidth\epsfbox{c1VSmassljetsCUTCOUNTy03.pdf}
\caption{The excluded region of ($c_1$, $m_X$) for a fixed set of $\xi$ and $y$. Two choices of $y$-values are shown. Left: $y=3$, corresponding to the case with $m_B \gg m_{5/3}$. Right: $y=0.3$, corresponding to the case with $m_B \gsim m_{5/3}$. For each of $y$-values, we plot the contours for three different values of $\xi \equiv (v/f)^2$: $\xi =0.1$ (dotted), $\xi =0.2$ (solid), and $\xi =0.4$ (dashed). Black lines are obtained by our ``$l$ + boosted tops/$W$s + jets'' style cut-and-count analysis, assuming 20 fb$^{-1}$ of LHC8 data. Red lines indicate the recasted CMS SSDL.}
\label{fig:c1vsMassOneLepton}
\end{center}
\end{figure}

Blah, blah, blah.....\\


The beautity of the single production process lies in that it has ability to probe the details of the strong dynames in composite Higgs model via the coupling constant in its production process. More abstract way of rephrasing is that the coupling constant in Eq.~\ref{eq:combine} can be written as
\beq
 g_X = g_X(\xi,\, y,\, c_1,\, c_2,\, m_X)~,
\eeq
where $\xi$, $y$, $c_{i=1,2}$, $m_X$ denote the set of parameters that defines the model and determines the spectra of top partners. While the exclusion curve in ($m_X$, $g_X$)-plane is able to present limits on top partners in more model-independent way, integrating in all differential effects of a bigger parameter space can provide us an alternative view of the status of certain underlying theories. 

As was explained in Section~\ref{sec:model}, one of the parameters, for instance $c_2$, can be removed by top mass. We show in \ref{fig:c1vsMassOneLepton} the excluded region of $c_1$ for varing top partner mass, given set of fixed $y$ and $\xi$. For the illustration we chose two values of $y$ representing two different mass hierarachies between $B$ and $X_{5/3}$ set by roughly ${\mathcal O}(yf)$
\footnote{In the composite Higgs models electroweak precision $S$ and $T$ parameters receive large corrections due to the nonlinearity of the Higgs boson, i.e. modification of its couplings to the $W, Z$, which translates into an overall bound on the scale of compositeness
\beq
 \xi < 0.1 \quad \Leftrightarrow \quad f>750\ {\rm GeV}~. \label{eq:nonlin}
\eeq
} as in Eq.~\ref{eq:Bmass}. For the case of $y = 3$, the contribution from $B$ is decoupled with respect to $m_{X_{5/3}}$ due to $m_B \gg m_{X_{5/3}}$. For small $y$, e.g. 0.3 in our choice in Fig.~\ref{fig:c1vsMassOneLepton}, the improvement by an additional contribution from $B$ is very significant. While we show the plots only for a few values of parameters, one can easily extract any plot for other choices of values from the set of contours in Figs.~\ref{fig:gVSmassLjets},~\ref{fig:dmVSmassLjets}. The parameters in Fig.~\ref{fig:c1vsMassOneLepton} also get constrained indirectly by the electroweak precision measurements (EWPM). For instance, a prohibitively large $S$ parameter can be generated by virtual exchanges of composite resonances through the interaction $c_1$, even without any mixing with elementary fermions, and it can be larger than the effects of the Higgs nonlinearity~Eq.\ref{eq:nonlin}[CITE:Barbieri]. This translates into a constraint on the $c_1$ parameter, which in the absence of cancellations cannot be very different from one, 
\beq
|c_1-1| \lesssim 0.2~.
\eeq
On the other hand, the $T$ parameter contrains $m_{5/3}$ through the mass relation with $X_{2/3}$ that can mix with the elementary particles and necessarily breaks the custodial symmetry. The bounds can be as strong as,
\beq
m_{X_{2/3}}\sim m_{X_{5/3}}\gtrsim 0.5-1 \hbox{ TeV}~,
\eeq
depending on whether there are cancellation in $S$ parameter.


%%%
% Where to put these ?
%%%

%At last we would like to mention a constraint arising from $b\rightarrow s\gamma$. This flavor violating decay can be enhanced via the operator
%\beq
%O_{Htb}=(\bar t_R \gamma^\mu b_R) H^* D_\mu H,
%\eeq
%where $O_{Htb}$ can be generated at tree level by exchange of the top and bottom partners and leads to the overall bound of {\bf msp: what is constraint here? Mass of top partner? Wilson coefficient of an operator? I think we need to be more precise.}
%\beq
%0.54-1\hbox{TeV}~,
%\eeq
%depending on the sign of the contribution~\cite{}. Note that this bound can be ameliorated by making the partners of the righthanded bottom quark much heavier.

